The Art of SOCRATIC QUESTIONING: Recursive Thinking with Large Language Models

Chain-of-Thought (CoT) prompting enables large language models to solve complex reasoning problems by generating intermediate steps. However, confined by its inherent single-pass and sequential generation process, CoT heavily relies on the initial decisions, causing errors in early steps to accumulate and impact the final answers. In contrast, humans adopt recursive thinking when tackling complex reasoning problems, i.e., iteratively breaking the original problem into approachable sub-problems and aggregating their answers to resolve the original one. Inspired by the human cognitive process, we propose SOCRATIC QUESTIONING, a divide-and-conquer style algorithm that mimics the recursive thinking process. Specifically, SOCRATIC QUESTIONING leverages large language models to raise and answer sub-questions until collecting enough information to tackle the original question. Unlike CoT, SOCRATIC QUESTIONING explicitly navigates the thinking space, stimulates effective recursive thinking, and is more robust towards errors in the thinking process. Extensive experiments on several complex reasoning tasks, including MMLU, MATH, LogiQA, and visual question-answering demonstrate significant performance improvements over the state-of-the-art prompting methods, such as CoT, and Tree-of-Thought. The qualitative analysis clearly shows that the intermediate reasoning steps elicited by SOCRATIC QUESTIONING are similar to humans' recursively thinking process of complex reasoning problems.

==> 1introduction_new.tex <==
\section{Introduction}
\begin{quote}
\textit{The art of Socratic Questioning is important for critical thinkers and excellence of thought. What Socratic adds is systematicity, depth, and a keen interest in assessing the plausibility of things.} 
\\
\centerline{- L. ELDER and R. PAUL, 1998}   
\end{quote}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/question_exp.pdf}
%     \caption{Example of a complex visual question solved in the human thinking process, involving raising \textcolor{visual_orange}{visual} and \textcolor{fact_pink}{commonsense} questions.\jy{another general example}jy{change the figure}}
%     \label{fig:question_exp}
% \end{figure}
\begin{figure}[th]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/intro_example.pdf}
    % \caption{test}
    \caption{Example of a complex language reasoning task solved by the Standard Prompting, Chain-of-Thought, and \method{}. Correct but helpless reasoning is highlighted in \textcolor{brown}{brown}, and incorrect reasoning is highlighted in \textcolor{red}{red}.\lifu{this is not a good example as the reason that CoT incorrectly answers the questions is that the last reasoning step was not correct instead of it doesn't know where to start; also, it cannot show the advantage of the Socratic Questioning - its reasoning is quite similar as CoT.}}
    \label{fig:question_exp}
\end{figure}
Humans are good at solving complex problems due to two significant capabilities: \textit{self-questioning}, meaning that we proactively ask questions from multi-angles that help elevate the understanding or solving of the target problem, and \textit{recursive thinking}, if the answer is not immediately achievable, we think more deeply by decomposing the complex problem into simpler and solvable sub-problems, recursively. 
% \zhiyang{change example Consider the image and question presented in Figure~\ref{fig:question_exp}; to derive the answer, an intelligent agent would proactively ask questions, such as \textit{What can make a balloon float?}, \textit{Why can a balloon float?}, \textit{What is the principle of objects floating?}, to delineate the implicit, necessary, additional information and knowledge from intermediate steps, until reaching the final answer, a full stopping signal.} 

\input{figures/overview_fig.tex}

Recently, by scaling up the parameters, large-scale language models (LLMs)~\cite{Brown2020GPT3, Chung2022FlanT5, ChatGPT, Touvron2023LLAMA} gain the capability of decomposing the complex problem and solving it step by step. Such emerging ability is called Chain-of-Thought (CoT)~\cite{wei2022COT} and it is proven to be effective on various complex reasoning tasks. However, CoT is a greedy thinking process that always starts with the first step of the task and continuously generates the next step based on previous steps. It only explores a single way of thinking to approach a problem and errors from previous steps can easily accumulate~\cite{Turpin2023CoTUnfaithful}. Self-Consistency of CoT (SC-CoT)~\cite{wang2022self} checks multiple paths of thinking but it is not efficient in exploring the thinking space, e.g., it is greedy after picking the starting point of a reasoning path\lifu{what does it mean}. The most recent Tree-of-Thought (ToT)~\cite{yao2023ToT} decomposes a question into small steps. At each step, multiple thoughts are proposed and only a set of promising thoughts are kept for further exploration.
% leverages tree-searching algorithms to efficiently find the optimal thinking path. However, it relies on the assumption that language models can estimate the value of the current state.
However, CoT, SC-CoT, and ToT only represent a limited form of the human thinking process, which starts with the most basic ideas or observations and  generalizes to the final conclusion step-by-step}.  However, in many complex reasoning tasks, even humans do not know where to start, and different starting points of thinking can lead to very different conclusions. Exploring the thinking space by trying each of the starting points is inefficient.
\minqian{I feel it can make reader easier to understand the "starting point" by very briefly providing an example of the starting point and how it may lead to different conclusions} \lifu{I agree with Minqian. The concept "starting point" is vague and it's better to provide an example. Also, are we really sure that CoT approaches must have a valid starting point? If the first step is not relevant to the target problem, but as it has a chain, is that possible that this chain may still have the correct first reasoning step and finally reach the correct answer?}

Inspired by the self-questioning and recursive thinking of humans, we propose \method{}, a novel divide-and-conquer fashion algorithm that simulates the top-down exploration and bottom-up backtracking process of a human, as shown in Figure~\ref{fig:overview}\lifu{it's very hard to imagine how it works by looking at Figure 2 at this stage as there is not concrete example shown in Figure 2. We need to either add concrete examples to Figure 2, or use the example in Figure 1 but it needs to show the }. In the top-down phase, \method{} recursively breaks a problem into simpler sub-problems until the sub-problems can be solved. In the bottom-up phase, the solutions to the sub-problems are returned and used to solve the original problem. We argue that \method{} represents a thinking process differing from CoT, the deductive reasoning, which starts from the conclusion and recursively seeks for premises to support the conclusion.\lifu{this is very difficult to interpret. I would recommend avoiding using deductive/inductive reasoning but stating the fundamental difference only}
% The input space of \method{} is a piece of text that clearly define a problem together with some context (e.g., images) and the output space is a textual answer to the problem. 
%The core component of \method{} is a Self-Questioning (SQ) module that leverages large-scale language models to 
The core component that drives \method{} is a \selfQuestion{} (SQ) module, that leverages large-scale language models to proactively raise and answer questions that are essential to solving the target question and can be viewed as intermediate reasoning steps. \method{} recursively backtracks and tailors intermediate thoughts acquired from \selfQuestion{} until reaching an answer to the original input question.
\minqian{I feel that it will be beneficial and more clear if we can summarize and highlight the key advantages of our method over CoT/SC-CoT/ToT with several bullet points. }

%a large-scale language model (LLM) which has three main functionalities: (1) dividing a problem into sub-problems, (2) deciding if a problem is answerable, and (3) generating answers. The three functionalities can be achieved by the same LLM with different task instructions.
To show the effectiveness of \method{}, we conduct extensive experiments on various complex reasoning tasks including the chemistry and physics tasks in the Massive Multitask Language Understanding~\cite{Hendrycks2020multitask}, mathematical tasks in the MATH dataset~\cite{Hendrycks2021math}, and reading comprehension in LogiQA~\cite{Liu2020logiqa}. Additionally, we showcase the generalizability of our method by conducting experiments with zero-shot visual question answering in VQA-V2~\cite{goyal2017making}, OK-VQA~\cite{okvqa}, and AOK-VQA~\cite{schwenk2022okvqa} datasets.
% In addition, we demonstrate our method can generalize to a more challenging setting by experimenting \method{} with zero-shot visual question answering in VQA-V2~\cite{goyal2017making}, OK-VQA~\cite{okvqa}, and AOK-VQA~\cite{schwenk2022okvqa}. In the experiment results, we observe that All of the tasks require strong
The experimental results show that
\method{} achieves significant performance improvement over CoT, SC-CoT, and ToT on all language tasks and outperforms several strong baselines in zero-shot VQA. The qualitative analysis also demonstrates that \method{} is capable of eliciting the intermediate reasoning steps through \selfQuestion{}, like a critical thinker, and solving complex reasoning problems.

\input{figures/comparison_fig}

% take zero-shot visual question answering (VQA) as a case study. This task is challenging because LLMs lack the capability to directly process the visual images, but instead, are expected to recursively acquire visual information and external knowledge that is necessary and beneficial to answer the input question. We evaluate \method{} on zero-shot VQA with three public benchmark datasets: VQA-V2~\cite{goyal2017making}, OK-VQA~\cite{okvqa}, and AOK-VQA~\cite{schwenk2022okvqa}. \method{} shows significant improvement over several strong baselines on (almost) all the datasets. The qualitative analysis also demonstrates that \method{} is capable of eliciting the intermediate reasoning steps through \selfQuestion{}, like a critical thinker, and solving complex reasoning problems.  

%, we clearly observe the novel ways of thinking a problem instigated by \method{}.\footnote{We will release the code upon acceptance.}  

% demonstrate strong performance improvement brought by \method{} on all of them. In our qualitative results, we clearly observe the novel ways of thinking a problem instigated by \method{}.\footnote{We will release the code upon acceptance.}  

%We provide an LLM with a \visualPercept{} module (\vlm{}) that can generate captions focusing on input prompts. 
%The information stored in an image is dense and in order to answer a visual question, the LLM needs to control the \vlm{} to explore the visual space of the image. Since the image is partially observed and the observations are noisy, the LLM needs to imagine missing information, think about the potential ways of solution, and plan the thinking paths approaching the problem.

% To summarize, we propose \method{}, a novel recursive algorithm based on self-questioning and recursive thinking of humans. We take zero-shot VQA as a case study and by evaluating our method on three public benchmark datasets: VQA-V2, OK-VQA, and AOK-VQA, we demonstrate strong performance improvement brought by \method{} on all of them. In our qualitative results, we clearly observe the novel ways of thinking a problem instigated by \method{}.\footnote{We will release the code upon acceptance.}






% Recent studies have shown that, by scaling up the parameters, large language models (LLMs) pre-trained on an enormous among of text corpora have excelled at numerous tasks and shown emerging capabilities, such as Chain-of-Thought (CoT) which performs multi-step reasoning by building intermediate steps. 
% However, as tasks increase in complexity and require more intermediate steps, the CoT approach faces challenges in performing a complete reasoning process\cite{kazemi2022lambada,wang2023plan}.
% Some critical steps are missed, resulting in an incomplete logical chain. Furthermore, it is uncertain whether CoT can accomplish information-intensive tasks through in-context learning from a limited number of demonstrations\cite{khot2022decomposed}. Moreover, the dependence on knowledge solely contained within a large language model (LLM) often gives rise to hallucinations in intermediate steps\cite{kazemi2022lambada}. \lifu{add limitations of CoT (advantages of our approach over CoT)}
% The original divide-and-conquer algorithm can only be applied to certain problems (e.g., it requires a way of breaking the problem into sub-problems). We propose to leverage strong reasoning and planning capabilities~\cite{} of an LLM to divide any problem into sub-problems and decide if the sub-problem can be solved. The original divide-and-conquer algorithm can only be applied to certain problems (e.g., it requires a way of breaking the problem into sub-problems).






==> 3method.tex <==
\section{Method}
% \subsection{Prompt Generation}

% based on the caption, the instruction, and the text input of the task,  ChatGPT generates multiple prompts (multiple thoughts) to query the vision-language model for more context and select visual tools to obtain more information.





% The newly obtained information is merged with previous image-context to form new image context. In the mean time, we allow ChatGPT to search on the internet to obtain factual knowledge. given the image context 



% \subsection{List of Visual Tools}

% Caption \\
% Conditioning Caption \\
% Object Detection \\
% Grounded Caption \\
% Visual Relationship (Scene Graph) \\
% OCR \\
% Counting \\
% Visual Entity Linking\\
% Visual Attribute\\
% referring expression generation 

% \subsection{Comprehensive Caption Generation}

% \subsection{Visual Tool Selection}

% \subsection{Visual Chain-of-Thought}

%\subsection{Task Formulation}
\subsection{\method{}}
% We mainly consider the vision-language reasoning tasks involving a single image with or without text. We denote the dataset corresponding to a task $t\in T$ as $\mathcal D^t=\{(q^t, m^t_j, y^t_j) \in \mathcal{Q}^t \times \mathcal M^t \times \mathcal Y^t\}_{j=1}^N$ where $q_j^t$ denotes the question for the  instance from the task $t$, $x^t_j$ denotes the input image with text if provided, and $y^t_j$ denotes the output of the instance. We formulate such tasks into a sequence-to-sequence generation task. Our goal is to develop a task-agnostic mapping function that tasks in 
% $I^t$ and $x^t_j$, and output $y^t_j$. Formally, the mapping function can be expressed as $f:\mathcal{X}^t\times\mathcal{I}^t\rightarrow\mathcal{Y}^t$. \lifu{it's not clear what is $I^t$, and it's better to define a symbol for the question, and hint, so that later we can consistently use them}
%We mainly consider the vision-language reasoning tasks involving a single image with or without text. We denote the dataset corresponding to a task $t\in T$ as $\mathcal D^t=\{(I^t, x^t_j, y^t_j) \in \mathcal{I}^t \times \mathcal X^t \times \mathcal Y^t\}_{j=1}^N$ where $I^t$ denotes the instruction for the task $t$, $x^t_j$ denotes the input image with text if provided, and $y^t_j$ denotes the output of the instance. We formulate such tasks into a sequence-to-sequence generation task. Our goal is to develop a task-agnostic mapping function that tasks in $I^t$ and $x^t_j$, and output $y^t_j$. Formally, the mapping function can be expressed as $f:\mathcal{X}^t\times\mathcal{I}^t\rightarrow\mathcal{Y}^t$.%\lifu{it's not clear what is $I^t$, and it's better to define a symbol for the question, and hint, so that later we can consistently use them}

%\subsection{Overall Architecture}

\begin{figure*}
    \centering
    \includegraphics[width=0.98\textwidth]{figures/overview_concept4.pdf}
    \caption{The overview of the \selfQuestion{} Algorithm.}%Overview of our \method{} framework. For each output of Task Module (TM) or Multi-path Visual Prompting (MP3), if it involves the special token "Lack of Information" (LoI), it is then fed to another MP3 (\textcolor{fig_red}{red} line) to get hints for the current question (unless the current depth, i.e., turn number, reaches the pre-set threshold). Otherwise, the question-answer pair will be rephrased (\textcolor{fig_yellow}{yellow} line) to a statement sentence and backpropagated (\textcolor{fig_blue}{blue} line) to the previous question's context as a hint. Best viewed in color.}
    \label{fig:selfq}
\end{figure*}

Figure~\ref{fig:overview} shows the overview of the \method{} approach, which is essentially a recursive thinking process involving a top-down exploration process (in black line) and a bottom-up backtracking process (in \textcolor{back_green}{green} line). The top-down exploration process proactively divides the question into simpler sub-questions. The bottom-up backtracking process recursively solves questions in which the answers to sub-questions are collected to solve the higher-level more complex questions.

In the beginning, we're given a target question $Q^0$, context \zhiyang{$C$ (if available)}, and an optional hint $H^0$. The hint is initially null but will be gradually updated and enriched as the recursive thinking process continues and the { \selfQuestion{} Module} acquires more and more relevant factual and visual information.

At every depth $d$, we employ the top-down exploration process by invoking the {\selfQuestion} ({\SQ}) module, which takes in the question $Q^{d}$, hint $H^d$, and \zhiyang{context $C$}. \selfQuestion{} either directly generates the answer $\tilde{A}^{d+1}$ for the  sub-question $Q^{d}$ \textbf{or} generate the updated hints $H^{d+1}$ along with a set of  sub-questions $\mathcal{Q}^{d+1}$ related to $Q^{d}$.
% For each question $Q^{d+1}_i \in \mathcal{Q}^{d+1}$, we recursively invoke the \method{} to obtain the answer statement $\tilde{H_i^{d+2}}$ to the input question $Q^{d+1}_i$.
If \selfQuestion{} can directly answer the sub-question $Q^{d}$, we append its answer $\tilde{H}^{d+1}$, otherwise, we continue the exploration process by looping through the set of newly generated sub-questions and input each question $Q^{d+1}_i$ along with hints $H^{d+1}$, and image $I$ to the \selfQuestion{} module.
% \zhiyang{jinyuan add symbols}
The bottom-up backtracking process starts when the \selfQuestion{} module outputs an answer $A$ to the input question. The answers $A$ to the sub-questions $\mathcal{Q}^{d+1}$ climb up the tree and update and enrich the hints $H^d$ in their parent question $Q^d_i$. This recursive process continues until we reach the tree's root, and the target question $Q^1_1$ is answered by $\tilde{H}^{2}$. We provide the pseudo-code of our proposed algorithm in Algorithm~\ref{alg:RMVP}.
\input{algorithms/socratic.tex}
% backtracking pass and add the answer as a hint to resolve its parent question
% the essentially breaks the original question $Q^0$ into simpler ones until the model believes it can solve these simpler questions. The answers to the simpler questions then follow the bottom-up backtracking process to  climb up the tree to update and enrich the hints. This recursive process continues until we reach the tree's root, and the target question is answered. 
% The {\tt Self-Questioning} module aims to seek more additional information by proactively and sequentially asking and answering a set of factual and visual questions that are related to the input and necessary to answer the original target question. The answering to each intermediate visual question follows the same recursive thinking process for the original target question.


% Figure~\ref{fig:overview} shows the overview of the \method{} approach, which is essentially a recursive thinking process: given a target question $q$, an image $m$, and an optional hint $h$\footnote{The hint is initially null but will be gradually updated and enriched as the recursive thinking process continues and the {\tt Self-Questioning Module} acquires more and more relevant factual and visual information.}, we first employ a {\tt Multimodal Reasoning} ({\tt MR}) module that takes in all the input information and either predicts a specific answer for the target question or \textit{Lack of Information}, indicating that the current input information is not enough to answer the question. If {\tt MR} outputs \textit{Lack of Information}, we further feed all the input information into a {\tt Self-Questioning} ({\tt SQ}) module to acquire more factual and visual information related to the input. We append the additional information acquired from {\tt SQ} to update the hint and repeat the whole process until the target question is answered. The {\tt Multimodal Reasoning} module is designed to answer the target question by interpreting the input image and optional hint. It consists of a visual perception model (i.e., BLIP2~\cite{Li2023BLIP2}) to generate a caption for the input image and a large textual pre-trained language model to predict the answer by taking the question, image caption as well as hint as the instruction of the reasoning task.  The {\tt Self-Questioning} module aims to seek more additional information by proactively and sequentially asking and answering a set of factual and visual questions that are related to the input and necessary to answer the original target question. The answering to each intermediate visual question follows the same recursive thinking process for the original target question.

%which generates prompts to query the VLM based on current context and task instruction; (2) a Factual Question Generation (\factualquestion) module which generates factual questions to query a knowledge base for commonsense and domain-specific knowledge; (3) a Task Module (\taskmodule) which first decides if the context is sufficient to perform the task. If not, the model will output \textit{lack of information}. If the task module can perform the task, it directly generates the predicted output; (4) A Visual Perception (\vlm) module with light vision-language understanding capability takes in language prompts and generates corresponding captions, and; (5) A Prompt-Answer Merging (\promptanswer) module that tasks in prompt and its answer and merges them into a statement. The \promptgenerate, \factualquestion, \taskmodule, and \promptanswer\ modules are all based on the same LLM and we use different prompts to guide the LLM to perform different tasks.

% Figure~\ref{fig:overview} shows the overview of the \method{} approach, which consists of five components: (1) A Visual Prompt Generation (\promptgenerate) module which generates prompts to query the VLM based on current context and task instruction; (2) a Factual Question Generation (\factualquestion) module which generates factual questions to query a knowledge base for commonsense and domain-specific knowledge; (3) a Task Module (\taskmodule) which first decides if the context is sufficient to perform the task. If not, the model will output \textit{lack of information}. If the task module can perform the task, it directly generates the predicted output; (4) A Visual Perception (\vlm) module with light vision-language understanding capability takes in language prompts and generates corresponding captions, and; (5) A Prompt-Answer Merging (\promptanswer) module that tasks in prompt and its answer and merges them into a statement. The \promptgenerate, \factualquestion, \taskmodule, and \promptanswer\ modules are all based on the same LLM and we use different prompts to guide the LLM to perform different tasks.

\subsection{\selfQuestion{}}
% \paragraph{Multi-Path Probing Prompting (MP3)} Figure~\ref{fig:FQG_temp} demonstrates the detailed step of the MP3 algorithm. First, \selfQuestion{} takes in the task instruction and context, and generates a set of $k$ factual questions via \factualquestion{}. Second, the KB module answers the factual questions and the PAM module merges the factual questions and answers to form factual statements. The factual statements are appended back to the input context and the \promptgenerate{} module takes in the task instruction and the new context, and generates $k$ probing prompts. Third, the \vlm{} generates a description of the image based on each of the probing prompts. Finally, we generate an answer for each of the visual prompts by providing the \taskmodule{} with the visual prompt, context, and image description corresponding to the visual prompt. If the TM decides it has enough information to perform the task, it outputs the answer. If the TM can not perform the task, it outputs "\textit{Lack of information}". We provide a pseudo-code of the MP3 algorithm in Algorithm~\ref{alg:MP3} 
\jy{change to general}Figure~\ref{fig:selfq} demonstrates the detailed step of the \selfQuestion{} algorithm. \selfQuestion{} algorithm takes in the question $Q^d_i$, image $I$, and hints $H^d$ (if it is available), to try to generate an answer $A$ via \MR{} module. There are two cases for the return of \MR{} module: (1) if $A$ is not the pre-defined special phrase \textit{"Lack of information"} $A_{LOF}$, answer $A$ then be incorporated with question $Q^d_i$ and transferred to a statement by \QAhint{} module (skip if depth $d$ = 1) as hint $\tilde{H^{d+1}}$. Hint $\tilde{H^{d+1}}$ is returned as the output of \selfQuestion{}. (2) If the \MR{} module fails to answer the given question $Q^d_i$ and return spefical phrase $A_{LOI}$, then \selfQuestion{} algorithm will raise help questions for more information. First, \FQG{} module takes $Q^d_i$, image $I$, and hints $H^d$ as input to raise several factual questions $Q_f$. $Q_f$ will be answered by a \FQA{} module with factual answers $A_f$. $Q_f$ and $A_f$ are incorporated and transferred to factual hints $H_f$ via \QAhint{} module. $H_f$ is appended to input hints $H^d$ to construct the updated hints $H^{d+1}$. Second, inputs of \selfQuestion{} algorithm and $H_f$ will be taken as input to a \visualQuestion{} module to raise $n$ visual questions $Q^{d+1}_1$, ..., $Q^{d+1}_n$. The combination of visual question $Q^{d+1}_i$ and updated hints $H^{d+1}$ is returned as the output of \selfQuestion{} algorithm in the case (2).  
% the KB module answers the factual questions and the PAM module merges the factual questions and answers to form factual statements. The factual statements are appended back to the input context and the \promptgenerate{} module takes in the task instruction and the new context, and generates $k$ probing prompts. Third, the \vlm{} generates a description of the image based on each of the probing prompts. Finally, we generate an answer for each of the visual prompts by providing the \taskmodule{} with the visual prompt, context, and image description corresponding to the visual prompt. If the TM decides it has enough information to perform the task, it outputs the answer. If the TM can not perform the task, it outputs "\textit{Lack of information}". 
\input{algorithms/self_question}
We provide a pseudo-code of the \selfQuestion{} algorithm in Algorithm~\ref{alg:self_question}.

\subsection{\multimodalReason{} (\MR{}) Module}
\jy{context get}
The \MR{} module aims to answer a visual question, either the target question or an intermediate question asked by the \selfQuestion{} module, based on the given image and an optional hint. We propose to leverage LLMs to answer visual questions since some of the visual questions are knowledge-demanding and LLMs are capable of storing commonsense and domain-specific knowledge and excel in complex reasoning tasks~\cite{Brown2020GPT3, Zhang2022OPT, wei2022COT, Touvron2023LLAMA}.
% \paragraph{Visual Perception} The information embedded in images is dense and inaccessible to LLMs. A generic caption does not necessarily capture the visual information required to perform the task. Thus, we employ a visual perception model, \lifu{specify which model is used here}, to describe the content of the image that is specifically related to the question. The input to XX\lifu{add} is an image $m$ and a text prompt $q$ to query part of the image and the output is a description of the part of the image related to the prompt denoted as $c$: \lifu{change VP to the specific model}
% \begin{equation}
%     c=\text{\vlm{}}(m,q).
% \end{equation}
%\paragraph{Answer Prediction} 
% In addition, recent studies have shown that finetuned language model can perform unseen tasks by following task instructions~\cite{Wei2022instruct}. 
We propose to transfer the reasoning capability of LLMs to answer complex visual questions by transforming the image into text. The information embedded in images is dense and inaccessible to LLMs. A generic caption does not necessarily capture the visual information required to answer the question. Thus, we first employ a visual perception model, \BLIP{}~\cite{Li2023BLIP2}, to describe the content of the image that is specific to the question. The input to \BLIP{} is an image $I$ and a text prompt $q$ to query part of the image and the output is a image caption $C^d_i$ describing of the part of the image related to the prompt: 
% \lifu{change VP to the specific model, did you use the hint if it's available, check if the description is matched with what you do}
\begin{equation*}
    C_{i}^{d}=\text{\BLIP{}}(I,q).
\end{equation*}

After transforming the image into a text description, we further employ an LLM (i.e., GPT-3) to predict the answer. Specifically, the input to the LLM consists of 
% \lifu{re-write the following paragraph, include all the details}
% The input to the Task Module (\taskmodule{}) is
the given question $Q^d_i$, image caption $C^d_i$, optional hints $H^d$, and a prompt $p_{\text{\MR{}}}$ carefully designed for \taskmodule{}. $H^d_i$ is a set of sentences containing the visual information of the image and commonsense knowledge related to the question. $p_{\text{\MR{}}}$ asks the LLM to follow the instruction and give the answer $A$ based on the image caption and hints. When the hints are available, $p_{\text{\MR{}}}$ asks the LLM to indicate the hints used in its reasoning process. If there is insufficient information to answer the question, the LLM must output a pre-defined special phrase "\textit{ Lack of information}" $A_{LOI}$. 
\begin{equation}
    A=\text{\taskmodule{}}(Q^d_i, C^d_i, H^d).
\end{equation}
The detailed $q$ and $p_{\text{\MR{}}}$ examples are presented in Appendix \ref{app:tm}.
% The input to the Task Module (\taskmodule{}) is the task-specific instruction $I^t$, the context $\mathcal{C}_j$, and a prompt $p_{\text{\MR{}}}$ carefully designed for \taskmodule{}. $\mathcal{C}_j$ is a set of sentences containing the visual information of the image and commonsense knowledge related to the task. $p_{\text{\MR{}}}$ asks the LLM to follow the instruction and perform the task based on the context and if there is not enough information to perform the task, the LLM needs to output "\textit{ lack of information}". 
% \begin{equation}
%     y^t_j=\text{\taskmodule{}}(I^t,\mathcal{C}_j,p_{\text{\MR{}}}).
% \end{equation}
% The detailed prompt examples are presented in Appendix \ref{app:tm}.


%\subsection{Self-Questioning Module} 



% \subsection{Task Module}
% Recent studies have shown that finetuned language model can perform unseen tasks by following task instructions~\cite{Wei2022instruct}. We propose to leverage such emerging capability of the LLM to perform novel multimodal tasks by transforming the image into text. The input to the Task Module (\taskmodule{}) is the task-specific instruction $I^t$, the context $\mathcal{C}_j$, and a prompt $p_{\text{\MR{}}}$ carefully designed for \taskmodule{}. $\mathcal{C}_j$ is a set of sentences containing the visual information of the image and commonsense knowledge related to the task. $p_{\text{\MR{}}}$ asks the LLM to follow the instruction and perform the task based on the context and if there is not enough information to perform the task, the LLM needs to output "\textit{ lack of information}". 
% \begin{equation}
%     y^t_j=\text{\taskmodule{}}(I^t,\mathcal{C}_j,p_{\text{\MR{}}}).
% \end{equation}
% The detailed prompt examples are presented in Appendix \ref{app:tm}.


\subsection{Factual Question Generation Module}
% The ability to engage in commonsense reasoning usually necessitates reliance on the support of both commonsense and factual knowledge. 
% When responding to a question, humans usually retrieve relevant background knowledge subconsciously in their minds and then perform inferences based on the given context and retrieved knowledge. 
Some of the multimodal tasks require commonsense or domain-specific knowledge. Although LLMs can store and retrieve knowledge from its parameter, they are prone to hallucination and the black-box retrieving process is hard to debug. Thus, to clearly understand the factual knowledge used to perform the task, we propose a Factual Question Generation (\FQG{}) module. Specifically, \FQG{} is an LLM with a prompt $p_\text{\FQG{}}$ asking the LLM to illustrate the reason and then generate factual questions related to the task. \FQG{} takes in the given question $Q^d_i$, image caption $C^d_i$, optional hints $H^d$, and generates a set of factual questions $\mathcal{Q}_f$. 

\begin{equation}
    \mathcal{Q}_f=\text{\FQG{}}(Q^d_i, C^d_i, H^d).
\end{equation}
The detailed prompt $p_\text{\FQG{}}$ examples are presented in Appendix \ref{app:fqg}.
% These generated questions are constrained to commonsense or factual questions. Furthermore, the proposed questions are designed to yield definitive, consensus, and unique answers.

% Our \factualquestion{} module is constructed upon the chatGPT. We pre-define the system as a "blind asker." and provide examples of deeper questions. For given task instruction \textit{I} and context \textit{C}, these inputs postpone the demonstration using a pre-set template. Owing to the robust in-context learning capabilities of large language models (LLMs), ChatGPT can generate high-quality factual questions, thereby enabling the exploration of background knowledge to support subsequent reasoning processes. Figure \ref{} illustrates the demonstration and template employed for generating factual questions.


\subsection{\factualanswer{} Module}
We propose to leverage LLM as a \factualanswer{} module for answering the factual questions $\mathcal{Q}_f$. Previous work~\cite{petroni2019languageModelasKnowledgeBase} has shown that language models can achieve competitive performance with traditional NLP methods in knowledge retrieval. The \FQA{} is an LLM with a prompt $p_\text{\FQA}$ asking it to generate the answer $\mathcal{A}_f$ for given factual questions. The input to \FQA{} is factual questions $\mathcal{Q}_f$ and the prompt $p_\text{\FQA}$.
\begin{equation}
    \mathcal{A}_f=\text{\FQA{}}(\mathcal{Q}_f).
\end{equation}
The detailed prompt $p_\text{\FQG{}}$ examples are presented in Appendix \ref{app:kb}.
% We merge the question with their answers $\mathcal{A}_f$ to form factual hints $\mathcal{H}_f$ via the \QAhint{} module. These factual hints are added to the input hints $H^d$. The detailed prompt examples are presented in Appendix \ref{app:kb}.



\subsection{\visualQuestion{} Module}
Previous methods \cite{Yang2022PICa, Zeng2022SocraticModels} only use the \BLIP{} once to obtain the images' primary visual content, including generic captions or object names.
% We use visual prompts to facilitate VLM to explore information in the image. Contemporary image captioning models are adept at generating high-quality captions that describe the primary event depicted in an image. 
However, the critical information necessary to perform a task may not always be included in the primary content. 
% When humans view an image, they usually first form a broad but coarse-grained understanding. Following this initial impression, humans will then pay more attention to the content related to the given question, facilitating the acquisition of the information required for a response. A typical method is making some hypothesis based on the question and their background knowledge, and demonstrating it by image content. 
To address this problem, we propose a \visualQuestion{} module (\VQG{}) that generates visual questions $\mathcal{Q}^{d+1}$ directing the \BLIP's attention toward image content strongly related to the task. Specifically, \VQG{} takes in the input question $Q^d$, hints $H^{d+1}$, image caption $C^d_i$ with a prompt $p_\text{\FQG{}}$ asking the LLM to illustrate the reason and then produces a set of visual questions $\mathcal{Q}^{d+1}$. These visual questions are designed to query the image content from different perspectives and require minimal reasoning capability. The \BLIP's responses to these prompts can provide useful visual information to address the original task.
\begin{equation}
    \mathcal{Q}^{d+1}=\text{\VQG{}}(Q^d, H^{d+1}, C^d_i).
\end{equation}
The detailed prompt $p_\text{\FQG{}}$ examples are presented in Appendix \ref{app:vpg}.


\subsection{\QAhint{} Module}
To make the hints $\tilde{H^{d+1}}$ and $\mathcal{H}_f$ provided to \multimodalReason{} in natural language, we use \QAhint{} (\QAtohint{}) module to integrate and rewrite the questions posed by \FQA{} and \VQG{} as well as their answers to statement sentences. Specifically, we feed the question $Q^d_i$, $\mathcal{Q}_f$ and their answer $A$, $\mathcal{H}_f$ to an LLM with prompt $p_{\text{QA2H}}$. The LLM is asked to rewrite the question to a statement sentence based on the answer.
\begin{equation}
    \tilde{H^{d+1}} = \QAtohint{}(Q^d_i, A)
\end{equation}
\begin{equation}
    \mathcal{H}_f = \QAtohint{}(\mathcal{Q}^f, \mathcal{A}_f)
\end{equation}
The detailed prompt $p_{\text{QA2H}}$ examples are presented in Appendix \ref{app:am}.

% Our Visual Prompt Generation (\promptgenerate{}) module is also based on ChatGPT, wherein we pre-define the system as a "commonsense question asker." We provide examples of visual prompts covering various aspects to chatGPT at the beginning. The task instruction \textit{I} and context \textit{C} is appended to follow the examples. LLM like chatGPT is able to emulate a cognitive process "what should I know to answer the question"-"what I already know"-"what question I should ask" and then generate rational and logical questions. These questions, or visual prompts, guide the VLM in uncovering more question-pertinent visual information. This supplementary visual data either corroborates or contradicts the background knowledge, thereby assisting in responding to the original question. Figure \ref{} showcases the demonstration and the template employed for the generation of visual prompts.

% \subsection{Visual Perception Module}
% % have moderate language and visual understanding capabilities.
% The information embedded in images is dense and inaccessible to LLMs. A generic caption does not necessarily capture the visual information required to perform the task. Thus, we need a \vlm{} that can describe the content of the image based on an input text prompt. The input to the \vlm{} is an image $x_j^t$ and a text prompt $q_{v_i}\in\mathcal{Q}_v$ to query part of the image and the output is a description of the part of the image related to the prompt denoted as $c_{v_i}$:
% \begin{equation}
%     c_{v_i}=\text{\vlm{}}(x_j^t,q_{v_i}).
% \end{equation}

% Two prominent strategies exist for integrating LLMs with images: 1) Refining the LLM through an adapter to allow image input, and 2) Transforming the image into text, which is subsequently interpretable by the LLM. We select the latter approach for modularity and explainability, employing an image captioning model to convert the input image into captions.
% Nonetheless, as previously indicated, the rich information inherent in an image is challenging to express in a single sentence. Advanced dense captioning models can generate detailed and comprehensive descriptions for all objects within images. This solution mitigates the issue of information scarcity but introduces considerable noise. The critical and requisite information for answering a given question is typically conveyed within one or two sentences. Dense captions provide exhaustive information, but excess information constitutes noise for our Task Module.
% Consequently,
% we leverage a text-aware visual language model to transform the visual information from images into text. In this work, we use Blip2 as the backbone of our VLM. Blip2 accommodates both text and image inputs, generating image captions of content strongly associated with the posed question.





% \begin{algorithm}[t]
% \caption{Multi-path Probing Prompting (MP3)}\label{alg:MP3}
% % \begin{algorithmic}
% \DontPrintSemicolon
% \KwIn{Task instruction $I$, Context $\mathcal{C}$, Must\_Answer}
% % Initialize context $\mathcal{C}=\{c\}$\;
% \KwOut{A set of visual prompt and answer pairs $\mathcal{V}$=\{($q_{v_1}$,$a_{v_1}$), ($q_{v_2}$,$a_{v_2}$), ($q_{v_3}$,$a_{v_3}$),...\}}
% \tcp{generate factual questions}
% $\mathcal{Q}_{f}$ $\leftarrow$ \factualquestion{}($I$,$\mathcal{C}$)\;
% % $\mathcal{A}_{f}$ = []\;
% % \tcp{add factual knowledge into the context}
% \For{each $q_{f}$ \in $\mathcal{Q}_{f}$ }{
%  $\mathcal{C}$.insert(PAM)\;
%  % $\mathcal{C}$ \leftarrow \mathcal{C} $\bigcup$ \{MA($q_{f}$, KB($q_{f}$))\}\;
% }
% \tcp{generate visual prompts}
% $\mathcal{Q}_{v}$ $\leftarrow$ \promptgenerate{}($I$,$\mathcal{C}$)\;
% $\mathcal{V}$=\{\} \;
% \For{each $q_{v_i}$ \in $\mathcal{Q}_{v}$ }{
% \tcp{query the \vlm{} to get new visual context}
% % $c_i$ $\leftarrow$ MA($q_{v_i}$, VLM($q_{v_i}$)) \;
% $c_i$ $\leftarrow$ \vlm{}($q_{v_i}$) \;
% %  % $\mathcal{C}$ \leftarrow \mathcal{C} \bigcup AM($q_{f}$, KB($q_{f}$))\;
% $a_{v_i}$ $\leftarrow$ TM($I$, $\mathcal{C}$ $\bigcup$ \{$c_i$\}, Must\_Answer)\;
% $\mathcal{V}$.insert(($q_{v_i}$,$a_{v_i}$))\;
% % $c$ = MA($q_{v}$, VLM($q_{v}$))\;
% }
% % \end{algorithmic}
% \end{algorithm}
% \begin{algorithm}[t]
% \caption{Self-consistent Chain-of-Thought (SC-CoT)}\label{alg:CoT}
% % \begin{algorithmic}
% \DontPrintSemicolon
% \KwIn{Task instruction $I$, Context $\mathcal{C}$, a set of new context $\mathcal{V}_c$, Must\_Answer}
% % Initialize context $\mathcal{C}=\{c\}$\;
% \KwOut{Result of the task $a_I$}
% $\mathcal{A}\leftarrow\{\}$\;
% \For{each $c_i$ \in \mathcal{V}_{c} }{
% % $c_i$ $\leftarrow$ MA($q_{v_i}$, VLM($q_{v_i}$)) \;
% % $c_i$ $\leftarrow$ VLM($q_{v_i}$) \;
% %  % $\mathcal{C}$ \leftarrow \mathcal{C} \bigcup AM($q_{f}$, KB($q_{f}$))\;
% $a_i$ $\leftarrow$ TM($I$, $\mathcal{C}$ $\bigcup$ \{$c_i$\}, Must\_Answer)\;
% $\mathcal{A}$ .insert($a_i$)\;
% % $c$ = MA($q_{v}$, VLM($q_{v}$))\;
% }
% \tcp{check chain-of-thought consistency}
% $a_I\leftarrow$ SC($\mathcal{A}$)\;
% return $a_I$
% % \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[t]
% \caption{\method{}}\label{alg:RMVP}
% % \begin{algorithmic}
% \KwIn{Task instruction $I$, Context $\mathcal{C}$, Max\_Depth, Max\_Turn, Curr\_Depth, Curr\_Turn}
% Must$\_$Answer $\leftarrow$ False\;
% \If{$Curr\_Depth=Max\_Depth$}
%     {Must$\_$Answer $\leftarrow$ True\;}
% \tcp{perform the task}
% $a_I\leftarrow$ \taskmodule{}($I$, $\mathcal{C}$, Must\_Answer)\;
% \If{$a_I\neq$"lack of information"}
%     {return $a_I$}
% \tcp{generate visual prompts and their answers}
% $\mathcal{V}\leftarrow$ MVP($I$, $\mathcal{C}$, Must$\_$Answer)\;
% % \tcp{add new visual information into context}
% $\mathcal{V}_c\leftarrow\{\}$\;
% \For{each ($q_{v_i}$,$a_{v_i}$) \in \mathcal{V}}{
%     \If{$a_{v_i}=$"lack of information"}
%     {\tcp{recursively get visual info}
%     $a_{v_i}\leftarrow \text{R-MVP}$($I$, $\mathcal{C}$, Max\_Depth, Max\_Turn, Curr\_Depth+1, Curr\_Turn)\;}
%     $\mathcal{V}_c$.insert(MA($q_{v_i}$,$a_{v_i}$))\;
% }
% $\mathcal{C}\leftarrow\mathcal{C}\bigcup\mathcal{V}_c$ \;
% Must$\_$Answer $\leftarrow$ False\;
% \If{$Curr\_Turn=Max\_Turn$}
%     {Must$\_$Answer $\leftarrow$ True\;}
% \tcp{compute a consistent result}
% $a_I\leftarrow$ SC-COT($I$, $\mathcal{C}$, $\mathcal{V}_c$, Must\_Answer)\;
% return $a_I$
% \end{algorithm}

% \begin{algorithm}[t]
% \caption{\method{}}\label{alg:RMVP}
% % \begin{algorithmic}
% \KwIn{Question $Q$, Hint $H$, Max\_Depth, Curr\_Depth}
% \KwOut{Result of the task $a_I$}
% Must$\_$Answer $\leftarrow$ False\;
% \If{$Curr\_Depth=Max\_Depth$}
%     {Must$\_$Answer $\leftarrow$ True\;}
% \tcp{perform the task}
% $a_I\leftarrow$ \taskmodule{}($I$, $\mathcal{C}$, Must\_Answer)\;
% \If{$a_I\neq$"lack of information"}
%     {return $a_I$}
% \tcp{generate visual prompts and their answers}
% $\mathcal{V}\leftarrow$ MVP($I$, $\mathcal{C}$, Must$\_$Answer)\;
% % \tcp{add new visual information into context}
% $\mathcal{V}_c\leftarrow\{\}$\;
% \For{each ($q_{v_i}$,$a_{v_i}$) \in \mathcal{V}}{
%     \If{$a_{v_i}=$"lack of information"}
%     {\tcp{recursively get visual info}
%     $a_{v_i}\leftarrow \text{R-MVP}$($I$, $\mathcal{C}$, Max\_Depth, Max\_Turn, Curr\_Depth+1, Curr\_Turn)\;}
%     $\mathcal{V}_c$.insert(MA($q_{v_i}$,$a_{v_i}$))\;
% }
% $\mathcal{C}\leftarrow\mathcal{C}\bigcup\mathcal{V}_c$ \;
% Must$\_$Answer $\leftarrow$ False\;
% \If{$Curr\_Turn=Max\_Turn$}
%     {Must$\_$Answer $\leftarrow$ True\;}
% \tcp{compute a consistent result}
% $a_I\leftarrow$ SC-COT($I$, $\mathcal{C}$, $\mathcal{V}_c$, Must\_Answer)\;
% return $a_I$
% \end{algorithm}
% Algorithm~\ref{alg:RMVP} summarizes the pseudo code for our proposed \method{} in the VQA setting. The input to the algorithm is a question $Q^0$ and some context, an image $I$ and  


% Due to the complication of the original task, sometimes even the probing prompt asks for high-level information about the image and can not be answered based on the description from the \vlm{}. In such a case, we need to further divide the probing prompt into simpler prompts querying more basic information about the image. Thus, we propose an algorithm \algoThree{} that recursively divides the original task into simpler probing prompts (tasks), and the answers to the simpler prompts are returned back as additional visual information to help perform higher-level tasks. The overall algorithm is shown in Figure~\ref{fig:overview}. The input to the algorithm is a task instruction, some context, max question depth, and max question turns. The base case is to check if the \taskmodule{} can predict the answer based on the context. If \taskmodule{} can predict the answer, the answer is returned. Note that the \taskmodule{} must predict the answer when max depth or max turn is reached. If \taskmodule{} outputs "\textit{Lack of information}", the task instruction together with context are passed into the \selfQuestion{} and \selfQuestion{} outputs $k$ probing prompts (line 9 in Algorithm~\ref{alg:RMVP}). Next, each of the probing prompts with the updated context from \selfQuestion{} is input into \algoThree{} and the probing prompt becomes a new task instruction. (line 11-15 in Algorithm~\ref{alg:RMVP}). We argue that each of the probing prompts represents a way of thinking about the original task, hence we append each visual hint to the context separately and input the parent task with the new context into the \taskmodule{}. We are able to collect $k$ answers corresponding to each visual hint. Finally, we select the most consistent answer via Algorithm~\ref{alg:CoT} as the final output.





==> 4experiment.tex <==


\section{Experiment Setups}

\subsection{Implementation Details}

% \lifu{update this paragraph after completing the approach section}
We use blip2-flan-t5-xl\footnote{\url{https://huggingface.co/Salesforce/blip2-flan-t5-xl}} as our \visualPercept{} module.
% The \BLIP{} model serves as the backbone for our visual language model, and we employ the officially released ``pretrain\_flant5xl'' (3B) checkpoint for the frozen LLM in \BLIP{}.
We leverage ChatGPT~\cite{ChatGPT} for \question{}, \answer{}, \factualquestion{}, \factualanswer{}, \visualQuestion{}, \QAhint{}, and \multimodalReason{}. While ChatGPT generally outperforms GPT-3, we opt to employ \texttt{GPT-3-davinci-003} in the \multimodalReason{} module to answer questions. This decision is motivated by the observation that ChatGPT tends to be excessively cautious and neutral, and avoids responding to some questions. We provide detailed sample prompts for each module in Appendix \ref{app:prompt}.

\subsection{Baselines}
\paragraph{chatGPT~\cite{brown2020language}} is a large-scale pre-trained language model that demonstrates strong zero-shot and in-context learning ability on many tasks in natural language processing. GPT-3 serves as the single-modality baseline that only accepts natural language as the input.
\paragraph{\BLIP{}~\cite{Li2023BLIP2}}  
% is a pre-training strategy that offers an efficient approach for vision-language representation learning. It leverages off-the-shelf frozen pre-trained image encoders and large language models to bridge the modality gap. BLIP-2 consists of two stages: the first stage focuses on vision-language representation learning, while the second stage focuses on vision-to-language generative learning.
% is a pre-trained visual language model. It leverages frozen pre-trained image encoders and large language models by a Transformer encoder, achieving state-of-the-art performance on vision-language tasks. In this work, we employ the released FLAN-T5-XL~\cite{Chung2022FlanT5} checkpoint for the \BLIP{} model.
is a pre-trained vision-language model that leverages an efficient and generic pre-training strategy and achieves state-of-the-art performance on various vision-language tasks. In this work, we employ the released FLAN-T5-XL~\cite{Chung2022FlanT5} checkpoint as the frozen LLM for \BLIP{}.

\paragraph{GPT-3~\cite{brown2020language}} is a large-scale pre-trained language model that demonstrates strong zero-shot and in-context learning ability on many tasks in natural language processing. GPT-3 serves as the single-modality baseline that only accepts natural language as the input.
% is an autoregressive language model that uses a decoder-only transformer network with 175 billion parameters. The model was trained using generative objectives and demonstrated strong zero-shot and few-shot learning on many tasks. 
We adopt \texttt{GPT-3-davinci-003} in our experiments.

\paragraph{PICa~\cite{Yang2022PICa}} is a multi-modality approach that prompts GPT-3 with image captions to solve VQA in an in-context learning manner. 
% Specifically, PICa converts the image into captions and then adapts GPT-3 to solve the VQA task by providing a few in-context VQA examples. 
In our experiments, we implement PICa by using \BLIP{} as the image captioning model to prompt \texttt{GPT-3-davinci-003} to perform the VQA tasks.

\subsection{Evaluation Metrics}
To assess the effectiveness of our framework, we employ the conventional VQA accuracy metric \cite{goyal2017making} and we term it as "Traditional VQA Accuracy". Besides, since the metric applies a stringent penalization for minor discrepancies in grammatical structure in answers, we incorporate additional ground-truth answers to mitigate potential limitations of this metric. Specifically, for noun-based ground-truth answers, we add their corresponding plural forms to the answer set. For verb-based ground-truth answers, we include their progressive tenses as answers. Note that the supplementary answer variants maintain an equivalent quantity to their original counterparts.
% \zhiyang{jingyuan add NLI based method}

In addition, to address the limitation due to synonyms and expression differences, we also employ a semantic-match-based accuracy. Specifically, we deploy a natural language inference (NLI) model to determine if the ground-truth answer and the model prediction have the same semantic meaning for a given question. For example, given an image of a person catching a Frisbee, to the question \textit{``Why is this person reaching out?''}, the prediction \textit{``to catch Frisbee''} should be regarded as the same as the ground truth \textit{"to catch"}. In this work, we use ChatGPT as the NLI model. We show the prompt used for ChatGPT in evaluation in Appendix \ref{app:grade}.

\subsection{Datasets}

\paragraph{VQA-V2~\cite{goyal2017making}}
is a dataset containing open-ended questions about images. We adopt its validation set for evaluation, where it includes over 40K real images and 2M corresponding question-answer pairs. One limitation of this dataset is that most questions are about simple visual recognition and they do not require much reasoning or external knowledge~\cite{okvqa}.
% The questions in VQA-V2 generally focus on the image content itself and require less inference

\paragraph{OK-VQA~\cite{okvqa}}
is a VQA dataset that requires methods to draw upon external knowledge to answer questions. We use the test split with over 5K question-answer pairs in our evaluation. 
% OK-VQA collects only questions that require external knowledge to answer 
% Questions in OK-VQA require the reasoning ability of a model to incorporate outside knowledge and infer the correct answer. 

\paragraph{AOK-VQA~\cite{schwenk2022okvqa}}
is an augmented successor of OK-VQA, which is also a knowledge-based VQA benchmark. We conduct the experiments on its validation dataset that includes over 1K questions. The questions in AOK-VQA require a diverse base of commonsense knowledge and performing some form of reasoning to obtain the answers.
% In addition, the questions of AOK-VQA usually cannot be answered by simply querying a knowledge base. It requires a stronger reasoning ability of a model to infer the relationship between outside knowledge and image content to answer questions.

\paragraph{Data Leakage in \BLIP{} and GPT-3} 
In our preliminary experiments, we discovered an issue that pre-trained models could be subject to data leakage during their pre-training stage. We observed that the baseline models (i.e., \BLIP{} and GPT-3) achieved unjustifiably high performance across all three VQA datasets even without taking images as inputs (see Table~\ref{tab:no_img}). 
%we applied a filtering mechanism to the testing sets under the "no image given" condition. Specifically, 
To address this issue, we applied a filtering process to remove such contaminated instances. We first test the \BLIP{} and GPT-3 on zero-shot VQA tasks while replacing the original input image with an image composed entirely of black pixels of the same size. Then, we only retain the samples where the models failed to yield a correct answer when the original image is not given. After the filtering, we adopt the 500, 462, and 444  test samples for VQA-V2, OK-VQA, and AOK-VQA, respectively. We use these clean examples for the evaluation throughout the rest of our experiments. 
% \minqian{double check this: I think we may also include a reason that some instances are ill-designed such that the question can be answered without using the image}

% ----- old version
% In our preliminary experiments, we discovered an issue with the data leakage of pre-trained models. We observed that the baseline models (i.e., \BLIP{} and GPT-3) achieved an unjustifiably high-performance level across all three VQA datasets without taking images as input (Table~\ref{tab:no_img}). To address this concern, %we applied a filtering mechanism to the testing sets under the "no image given" condition. Specifically, 
% we test the \BLIP{} and GPT-3 on zero-shot VQA tasks while replacing the input image with a pure black image of the same size, and only retain the samples that yielded negative outcomes. In this way, we only use 500, 462 and 444 test samples for VQA-V2, OK-VQA and AOK-VQA, respectively, for evaluation.

\begin{table}[h]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{c|c|c|c}
\toprule \toprule
\textbf{Model} & \textbf{VQA-V2} & \textbf{OK-VQA} & \textbf{AOK-VQA} \\ \midrule
\BLIP{}          & 1.46            & 2.93            & 28.08            \\
GPT-3   & 35.88           & 23.95           & 20.4            \\ \bottomrule \bottomrule
\end{tabular}
}
\caption{Traditional VQA Accuracy (\%) under the setting where no image is provided in the input.} 
\label{tab:no_img}
\end{table}

% In order to avoid the effect of data-leaking in GPT-3 and \BLIP{} (Section \ref{sec: data-leak}), for experiments whose results are presented in this paper, we filter and remain 500, 462 and 444 test samples for VQA-V2, OK-VQA and AOK-VQA, respectively.




% \subsection{Zero-Shot VQA}
% VQA-V2\\
% OK-VQA \\
% AOK-VQA \\
% GQA \\
% Grounded VQA\\


% \begin{table*}[ht!]
% \scriptsize
% %\setlength\tabcolsep{11pt}
% \begin{center}
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{l | c  c | c  c  c  c c  c}
% \toprule
%  Models & Trainable Params & Total Params & VQAv2 & OK-VQA & GQA & Grounded-VQA & Text-VQA \\
% \BLIP{} & 224M & 269M & \\
% ChatGPT \\
% BLIP2 + ChatGPT & 224M & 269M & \\
% LM-Eyes & 224M & 269M & \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \vspace{-0.4cm}
% \caption{
% }
% \label{tab:zs_VQA}
% \vspace{-3mm}
% \end{table*} 

% \subsection{Zero-Shot Multimodal QA}
% Science-VQA \\
% MuMu-QA \\
% WebQA \\

% \begin{table*}[ht!]
% \scriptsize
% %\setlength\tabcolsep{11pt}
% \begin{center}
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{l | c  c | c  c  c  c c  c}
% \toprule
%  Models & Trainable Params & Total Params & ScienceQA & WebQA & MuMuQA \\
%  & \\ 
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \vspace{-0.4cm}
% \caption{
% }
% \label{tab:zs_VQA}
% \vspace{-3mm}
% \end{table*} 

% \subsection{Zero-Shot Multi-Modal Commonsense Reasoning}
% Visual Entailment \\
% NLVR \\
% Visual-Spatial Reasoning \\
% Commonsense VQA \\



% \begin{table*}[ht!]
% \scriptsize
% %\setlength\tabcolsep{11pt}
% \begin{center}
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{l | c  c | c  c  c  c c c}
% \toprule
%  Models & Trainable Params & Total Params & VCR & VCR-Exp & VSR & Visual Entailment & NLVR & NLVR2 & \\
% VL-T5_{} & 224M & 269M & \\ 
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \vspace{-0.4cm}
% \caption{
% }
% \label{tab:zs_VQA}
% \vspace{-3mm}
% \end{table*} 

% \subsection{Zero-Shot Multi-Modal Miscellaneous Tasks}

% Multimodal Factual Checking \\
% Multimodal Event Extraction \\
% Disaster classification \\
% Hateful Content Classification \\



==> 5discussion.tex <==
\section{Results and Discussions}
\begin{figure*}[ht!]
    \includegraphics[width=0.9\textwidth]{figures/textresult_detail.pdf}
    \caption{Selected examples of few-shot text reasoning task using the CoT and \method{}. \minqian{typo: "Tree-of-Thought"; we also need to specify which answer is correct for each question}}%\lifu{update the approach name in the figure}}
    \label{fig:textresult_exp}
\end{figure*}
\subsection{Quantitative Results}
Table \ref{tab:result_text} shows the quantitative results using traditional accuracy for language-only tasks. From the table, we can find that compared with other more general approaches, the ToT framework does not work well in this step-unknown kind of task. For our \method{} method, simply increasing the maximum turn number does not improve the performance of Socratic Questioning method consistently. One reason is the overconfidence of the self-evaluation of the ChatGPT. In our framework, whether to conduct deeper or multiple turns of thinking is at the LLM's own discretion. When we relax the limit on the maximum number of iterations, the model still decide to end the thinking process and retuan a confident answer in the second turn. However, in both directly answer (DA) and multiple-choice cases, our \method{} method still reaches the best performance. Compared with the state-of-art approach, our method increases the accuracy in 4.34\%, 2.98\%, 4.22\%, 4.66\% in math, physics, chemistry, and logic questions, separately. 

Table \ref{tab:result_em} and \ref{tab:result_sm} show the quantitative results using traditional VQA accuracy and semantic-based accuracy, respectively. 
For both results, our \method{} method outperforms the previous state-of-the-art approaches in most cases, often by a large margin. The only exception is semantic-based accuracy on the VQA-V2 dataset. A possible reason is that the VQA task on VQA-V2 focuses more on the visual recognition and detection aspect and does not require much reasoning capability and external knowledge. Approaches relying on the image caption model will lose some information in the process of image-to-text transformation. In contrast, \BLIP{}, which directly takes the original image as input, has more advantages in identifying image content and thus performs better in the tasks that do not focus on benchmarking reasoning ability.

On the other datasets OK-VQA and AOK-VQA that require more outside knowledge and require reasoning capability, our \method{} outperforms both baselines. Compared with traditional VQA accuracy, improvement brought by our method is more significant in the semantic-based accuracy. There are two reasons: (1) With richer and more fine-grained information, the answers generated by \method{} are usually more complete and comprehensive. For example, for the ground-truth answer \textit{table}, the answer given by our framework is ``brown wood table in the center of the room'', which matches the image content and is more detailed. In this case, this answer will be considered as \textit{correct} in semantic-based evaluation but getting a zero-score in the traditional evaluation. (2) Traditional evaluation metrics often over-penalize the minor surface differences (e.g., \textit{rain} and \textit{raining}, \textit{sushi roll} and \textit{sushi rolls}). Semantic-based evaluation method, however, is not limited by this problem.

\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule\toprule
\multicolumn{1}{l|}{}  & \textbf{Math(DA)} & \textbf{Physics} & \textbf{Chemistry} & \textbf{LogiQA} \\\midrule
\textbf{Sd-Prompting}       & 7.00            & 65.11          & 53.20              & 54.67           \\
\textbf{CoT}           & 7.33            & 67.66          & 57.14              & 48.33           \\
\textbf{SC-CoT}           & 7.00            & 68.51          & 59.33              & 49.00           \\
\textbf{ToT}           & 0.00            & 40.00       & 26.60              & 22.22           \\
\textbf{Socratic(522)} & \underline{7.67}   & \textbf{71.49} & 63.55              & \textbf{59.33}  \\
\textbf{Socratic(532)} & \textbf{11.67}            & \underline{69.36}          & \textbf{63.55}     & \underline{58.00}          \\\bottomrule\bottomrule
\end{tabular}
}
\caption{Accuracy (\%) based on Exactly Match. The best performance is highlighted in \textbf{bold} and the second best performance is highlighted with \underline{underline}. } 
\label{tab:result_text}
\end{table}


\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{c|ccc}
\toprule \toprule
\textbf{Model} & \textbf{VQA-V2} & \textbf{OK-VQA} & \textbf{AOK-VQA} \\ \midrule
\BLIP{}                     & 36.7            & 21.14           & 0                \\
PCIa                     & \underline{43.18}     & \underline{29.94}     & \underline{28.6}       \\
SOCRATIC (Ours)       & \textbf{46.64}  & \textbf{31.24}  & \textbf{29.58}   \\ \bottomrule \bottomrule
\end{tabular}
}
\caption{Traditional VQA Accuracy (\%) based on Exactly Match. The best performance is highlighted in \textbf{bold} and the second best performance is highlighted with \underline{underline}. } 
\label{tab:result_em}
\end{table}

\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{c|ccc}
\toprule \toprule
\textbf{Model}  & \textbf{VQA-V2} & \textbf{OK-VQA} & \textbf{AOK-VQA} \\ \midrule
\BLIP{}                     & \textbf{57.2}            & 46.75           & 43.29                \\
PCIa                     & 49.8     & \underline{48.05}     & \underline{46.85}       \\
SOCRATIC (Ours)                    & \underline{54.4}  & \textbf{53.03}  & \textbf{49.55}   \\ \bottomrule \bottomrule
\end{tabular}
}
\caption{Semantic-based VQA Accuracy (\%) using NLI. The best performance is highlighted in \textbf{bold} and the second best performance is highlighted with \underline{underline}.} 
\label{tab:result_sm}
\end{table}

% \section{Discussions}


\begin{figure*}[h]
    \includegraphics[width=0.98\textwidth]{figures/result_exp.pdf}
    \caption{Selected examples of zero-shot VQA using \BLIP{} and \method{} (1-Depth 1-Turn, 2-Depth 2-Turn).}%\lifu{update the approach name in the figure}}
    \label{fig:result_exp}
\end{figure*}


\begin{figure*}[th]
    \includegraphics[width=0.98\textwidth]{figures/result_detail.pdf}
    \caption{Visualization of a complete recursive thinking process of \method{} (2-Depth 2-Turn). The process is initialized on the left and is continued on the right.}
    \label{fig:result_detail}
\end{figure*}

% \subsection{Data-leakage in ChatGPT and \BLIP{}}
% \label{sec: data-leak}
% In our preliminary experiments, we discovered an issue pertaining to data leakage. We observed that the baseline models achieved an unjustifiably high-performance level across all three VQA datasets without taking images as input (Table~\ref{tab:no_img}). To address this concern, %we applied a filtering mechanism to the testing sets under the "no image given" condition. Specifically, 
% we test the \BLIP{} and GPT-3 on zero-shot VQA tasks while replacing the input image with a pure black image of the same size, and only retain the samples that yielded negative outcomes. 

% \begin{table}[h]
% \centering
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{c|c|c|c}
% \toprule \toprule
% \textbf{Model} & \textbf{VQA-V2} & \textbf{OK-VQA} & \textbf{A-OKVQA} \\ \midrule
% \BLIP{}          & 1.46            & 2.93            & 28.08            \\
% GPT-3   & 35.88           & 23.95           & 20.4            \\ \bottomrule \bottomrule
% \end{tabular}
% }
% \caption{Traditional VQA accuracy (\%) under the setting where no images are provided as input.} 
% \label{tab:no_img}
% \end{table}

% \subsection{Effect of More Comprehensive Caption}

% \subsection{Effect of Visual Modules}

% \subsection{Visual Tool Selection}

% \subsection{Visual Chain-of-Thought}




\subsection{Case Study}
% \subsection{Active fine-grained information acquisition by \method{}}
Figure~\ref{fig:result_exp} shows several examples of few-shot language-only reasoning tasks based on the baselines and the \method{}. For the example question 1, CoT and ToT generate the reasoning process with some hallucination. Due to the one-direction generation nature of these two approach, LLMs do not have chance to self-chech and correct the potential hallucination which is obvious and easy to address. On the other hand, In the case of unconfident of answer, our method generates a few simpler question to seek more background knowledge to support its reasoning. Comparing with generating the explanation and answer at once, split and answer the sub-question individually is easier for LLM and reduce the probability of hallucination. Similarly, in the example question 2, incorrect calculation cannot be fixed in the baseline methods. In addition, we find that information in input is easier to prompt LLMs and more helpful than information generated during reasoning. In example question 2, the LLMs notice the stoichiometry ratio when the reaction equation is given as input. However it ignore the ratio when the equation is generated during the reasoning process, and therefore generate an incorrect equation. Example question 3 demonstrates the advantage of our \method{} when the starting point of reasoning is not clear. The baseline methods may generate some reasoning which is correct, related to question context, but helpless to solve question. That is because these baseline methods always require a starting point and start from the question context information. They tend to generate information related to these context first, then toward to answer step by step. When the starting point is is unclear, it will lead to helpless reasoing that is noise to LLMs. On the other hand, the \method{} method calls QG module to generate related question that helps to determine the key point of solving questions. The questions asking for key point help LLMs avoid reasoning on unnecessary direction, making the reasoning of LLMs more refine and robust.

Figure~\ref{fig:result_exp} shows several examples of zero-shot VQA tasks based on the baselines and the \method{}. For the example in the first line in the figure, the answer from \BLIP{} is irrelevant to the given question, suggesting that the natural language understanding and reasoning capabilities of current VLMs are not robust enough on zero-shot multimodal reasoning tasks. 
Besides, we observe that without the ability to actively decompose a complex problem into solvable sub-parts, the existing multimodal approaches often fail to perform complex reasoning that requires probing the fine-grained evidence presented in the image and are heavily limited by the descriptive ability of the image captioning model.
In the example in the third line in Figure~\ref{fig:result_exp}, PICa can only relies on a general description of the image \textit{"A man sitting on a chair talking on a cell phone."} and misses the details, i.e., \textit{the ashtray full of cigarette butt} which is critical to answering the question. In contrast, our approach proactively seeks the hints that are potentially helpful to the task, performs recursive reasoning on the collected hint (i.e., \textit{"There is smoking-related objects on the table."}), and finally predicts the correct answer. This example clearly demonstrates the superiority of our \method{} approach over existing methods. We also show the visualization of the recursive thinking process in Appendix~\ref{app:thinking}.

% --- old version
% Besides, we notice that the strategy of passively accepting VLM input\lifu{not clear} limits the performance of PICa on problems requiring fine-grained reasoning. This static kind of information acquists\lifu{not clear} relies entirely on the quality of image captioning. When the information is not involved in the main event of the image\lifu{not clear}, PICa is hard to obtain enough meaningful information for reasoning and inferring. 
% In contrast, the \method{} proactively and recursively acquires additional factual and visual information that is related to and benefits the answering of the target question, until the final answer is achieved. Compared with the static information strategy used in baselines, our dynamic information acquists can deal with more complex tasks and is more robust to various questions\lifu{need improvement}. 



%\lifu{vefiry this paragraph}\minqian{verified}




%determine what commonsense knowledge is required and raise factual questions to obtain corresponding responses. Based on commonsense knowledge, LLM can then raise visual prompts to guide VLM to focus on specific image content and extract more fine-grained image information. In this example, given the question \textit{"Why are the children wearing hats?"}, the LLM first determines the general reasons for "wearing hats". Then it guides the VLM to explore information related to each reason, including "sun position" and "temperature", etc. After incorporating the commonsense knowledge \textit{"cold weather makes people wear hats"} and visual information \textit{"it is cold"}, the model finalizes the answer \textit{"Warmth"}.


% \subsection{Language Model Inner monologue}

% \subsection{Effect of language Models}


% \subsection{Real-World User Experience}

% \subsection{Generation of Visual Tools}



==> algorithms/1introduction.tex <==
\section{Introduction}

Recent advances in vision-language pretraining~\cite{Radford2021CLIP, OFA2022Wang, Alayrac2022Flamningo, Wang2022BEiT3, Li2022BLIP, Li2023BLIP2} and multimodal instruction tuning~\cite{xu2022multiinstruct} have equipped Vision-Language Models (VLMs) with strong zero-shot capabilities. However, due to the specific domain of the pre-training data  (e.g., image-text pairs from the internet), the visual-language models lack the ability to perform complex reasoning tasks~\cite{Zeng2022SocraticModels}.  In addition, most of the VLMs can only process a single image per input, which prevents in-context learning and limits the diversity of input format. Large-scale Language Models (LLMs) pre-trained on diverse internet text data, on the other hand, are capable of storing commonsense knowledge and excel in complex reasoning tasks~\cite{Brown2020GPT3, Zhang2022OPT, wei2022COT, Touvron2023LLAMA} but lack the ability to process visual information. In this work, we study the problem of \textit{how to effectively leverage the strong chain-of-thought reasoning capability and in-context learning capability of LLMs to perform diverse complex visual reasoning tasks without training.} 
% which require the model to observe the visual content of the image, search for domain-specific or commonsense knowledge and perform chain-of-thought reasoning. 

Previously there are two main lines of work adopting the reasoning capability in LLMs to visual tasks. One line of works~\cite{Li2023BLIP2, Zhang2023LLAMA-Adapter} proposes to align the pre-trained LLMs~\cite{Chung2022FlanT5, Zhang2022OPT} with the vision models~\cite{Dosovitskiy2021ViT, Radford2021CLIP} via cross-attention~\cite{Li2023BLIP2} or additional perception modules~\cite{Alayrac2022Flamningo}. However, such approaches usually require a large amount of parallel image-text data for pre-training and task-specific data for fine-tuning. If one wants to utilize newly developed pre-trained models, the VLM needs to be trained from scratch. Another line of work tries to bridge LLMs with vision models via human language. For example, PICa~\cite{Yang2022PICa} feeds image captions as context to GPT-3 for a few-shot knowledge-based VQA and Socratic models~\cite{Zeng2022SocraticModels} utilize a VLM to detect various basic visual concepts (e.g., objects, place, and the number of people) and fill them into pre-defined templates for zero-shot image captioning. However, considering the density of the information embedded in an image, a generic caption may not capture the key information required to perform a specific task.  In addition, the Socratic models heavily rely on pre-defined language templates and there is only a single-step interaction between the LLM and the VLM. Both models passively receive visual information, which is different from how humans perceive the world and does not take the noises in the observations from the VLMs into account.
% and elicit novel multimodal capabilities
% \minqian{can consider drawing a teaser figure to concisely present the high-level idea}


To address the aforementioned problems, we propose \method{}, \textit{a multi-turn interactive framework that stitches vision and language models to cooperatively perform complex visual reasoning tasks without training while enjoying high transparency}. Specifically, \method{} is a form of cooperative argumentative dialogue \ying{cite/footnote/.. to explain cooperative argumentative dialog (From wiki: The Socratic method (also known as method of Elenchus, elenctic method, or Socratic debate) is a form of cooperative argumentative dialogue between individuals, based on asking and answering questions to stimulate critical thinking and to draw out ideas and underlying presuppositions.)} between an LLM and VLMs, instigated by the continual probing prompts of the LLM.
\zhiyang{rewrite such that we first say one step and then we say this step will repeat recursively.}
The dialogue structure in \method{} is a 1-ary tree \ying{1-ary??} and each node stores a task instruction and some context about the image. 
\ying{why not combine the following two paragraph to describe the k-ary socratic question in the first place, the intro seems too long}
\ying{ref to figure} In the beginning, the root node contains the original task instruction and a generic caption about the image, and the LLM tries to predict the answer for the task. If the LLM decides there is not enough information, it generates a probing prompt based on the task instruction and current context. By prompt engineering, we form a probing prompt such that it requires less high-level reasoning and more low-level awareness to be answered. A child node is initialized with the probing prompt as its task instruction. We query a VLM with the probing prompt to obtain a description for part of the image related to the prompt and append it to the context in the parent node to form the new context for the child node. The LLM now tries to answer the probing prompt in the child node and if it can not answer the probing prompt, the child node becomes the parent node and initializes its child node by generating an even more basic probing prompt.  If the LLM can answer the probing prompt, the answer and the prompt are combined to form a statement, and the statement is appended to the context in the parent node. The LLM tries again to perform the task in the parent node. If the task can not be performed even with the new statement, our method starts the second turn and initiates a new child node from the root node.

To alleviate the noises in the observations of the VLMs, we leverage the self-consistency of the Chain-of-Thought (SC-CoT)~\cite{Wang2022cot} method. Instead of generating a single probing prompt, we propose to generate $k$ prompts and initialize $k$ child nodes. This means the dialogue structure becomes a $k$-ary tree. Each child node represents a way of thinking to approach the parent task. After the $k$ child nodes return $k$ statements, the LLM addresses the parent task by considering each of the statements separately and draws $k$ answers. We then select the most consistent answer by marginalizing out the sampled reasoning path~\cite{Wang2022cot}.


To summarize, we propose \method{}, a novel framework that enables cooperative argumentative dialogue between an LLM and a VLM to perform complex visual reasoning tasks. \method{} addresses the oversimplified single-step interaction between the LLM and the VLM in previous work and allows the language model to explore the visual content via probing prompts. We evaluate our method on three public benchmark datasets: VQA-V2, OK-VQA, and AOK-VQA, and demonstrate strong performance improvement brought by \method{} on all of them. In our qualitative results, we clearly observe the entire thinking and decision-making process of the LLM, which proves the full transparency of our proposed method.\footnote{We will release the code upon acceptance.} 




% multiple china of the thought to the original question and they should be consistent multiview of the original question
% are two lady friends -> do they walk closer to each other, do they wear the same cloth, 
% low level visual information
% to query a VLM. The VLM returns visual information related to the prompt and the LLM tries to answer the generated prompt based on the original context together with the new visual information. If the LLM decides 
% this method closely emsembles the argumentative dialogue and critical thinking process between socratc and his students.
% To simulate the of multiple belief, we  
% We view the LLM as the human brain which can control and process the visual information obtained via VLMs (eyes). Given the task instruction and a generic caption of an image as the initial context, the LLM tries to perform the task. If the LLM decides it can not perform the task based on given visual information, it will automatically generate a list of prompts to prompt the VLMs. In such a way, the original task is divided into multiple sub-tasks.    
% If the task reuires more the continuesly generate visual prompts to collect more visual information. 
% allows LLMs to continuously prompt the VLMs for task-related visual information and address the incomplete and noisy observations from the VLMs. 
% \method{} consists of four modules: (1) A visual-prompt-generation (VPG) module which generates prompts to query the VLMs based on current information and task requirement; (2) a factual-question-generation (FPG) module which generates factual questions to query a knowledge base for commonsense and domain-specific knowledge; (3) a task module (TM) which first decides if the context is sufficient to perform the task. If not, the model will output \textit{lack of information}. If the task module can perform the task, it directly generates the predicted output; (4) A vision-language model with light visual reasoning capability takes in language prompts and generates corresponding captions.

% RMVP recursively generates prompts to query the VLM for obtaining visual information and we consider each prompt as one chain of thought. [To Be continued...]

\begin{figure*}
    \centering
    \includegraphics[width=0.98\textwidth]{figures/overview_concept4.pdf}
    \caption{Self-Questioning Algorithm}%Overview of our \method{} framework. For each output of Task Module (TM) or Multi-path Visual Prompting (MP3), if it involves the special token "Lack of Information" (LoI), it is then fed to another MP3 (\textcolor{fig_red}{red} line) to get hints for the current question (unless the current depth, i.e., turn number, reaches the pre-set threshold). Otherwise, the question-answer pair will be rephrased (\textcolor{fig_yellow}{yellow} line) to a statement sentence and backpropagated (\textcolor{fig_blue}{blue} line) to the previous question's context as a hint. Best viewed in color.}
    \label{fig:selfq}
\end{figure*}
% RMVP recursively generates prompts to query the VLM for obtaining visual information and we consider each prompt as one chain of thought. [To Be continued...]
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/mvp.pdf}
%     \caption{Illustration of Multi-path Visual Prompting (MP3) module.}
%     \label{fig:FQG_temp}
% \end{figure}
% The initial input to RMVP is the task instruction and a generic caption from the VLM as context. The task module attempts to complete the task based on the context. If the output from the task module is \textit{lack of information}, the factual-question-generation module takes in the context and task instruction and generates a group of factual questions to query a knowledge base. The answers along with the factual questions are merged into context. Next, the visual-prompt-generation module takes in the context and task instruction and generates $C$ prompts to query the vision language model.  





% while enjoy high transparency and interpretability.

% % based on the instruction and the context extracted from the image. The task module also decides if it can perform The input to RMP is the task instruction and a generic caption $C$ of the image. If the task module decides if it can successfully perform the task based on $C$, the task model directly generates the output. If the task module decides, it can not perform the task, the VPG raises K prompts where K is a hyper-parameter to query the VLM.  


% . the language model can actiavely ask for more visual infomrations and fact information. 




% propose by performing cooperative and argumentive dialogue between a LM and a visual-language model. However, considering the density of information in an image, the generic caption can not capture the detailed semantics of the image. When performing reasoning on an image, humans focus on the visual information that is related to the task. One can think of this process as generating the most plausible output based on incomplete and noisy observations. The LM continuously raises queries in different granularity to prompt the visual-language model to obtain more visual information. 


% We first provide a generic caption of the image to the LM. Then the LM performs the visual reasoning task based on the caption. If the caption does not contain enough information, the language model raises multiple queries to prompt the visual-language model to collect more visual information. 




% Motivation: \\
% 1. tasks require commonsense reasoning and external knowledge remains challenging.
% 2. pre-trained vision-language models are restricted to a single image and most of them are not able to perform tasks related to bounding boxes.\\
% 3. aligned vision-language models are less capable of following instructions.\\
% the visual-language model has some capability of performing simple visual tasks such as caption, VQA and describing part of the image based on a prompt. and we offload the reasoning process to the language model.


% Method:\\
% Group of visual tools\\
% multi-turn multi-path reasoning (MTMP)\\

% contribution:\\
% strong zero-shot capability on various multimodal tasks.\\
% great flexibility in terms of domain and task adaptation and easily registering new visual modules.\\
% propose multi-turn multi-path reasoning which is interpretable and makes the model easy to debug. \\
% demonstrate the language model can understand the task and automatically select the visual tools to finish the task.\\



% we provide a caption of the image as the initial context and allow the model to continuously prompt the visual model to obtain useful information and use visual tools. This process elicits explicit reasoning process and enable 


% The visual argument made by and language model needs to generate the most likely answer or explanation based on incomplete and noisy observations. If the language model is not confident about . the infomration exchange between lagnuage model and the visual-langugae model simulates the Socratic method which is a form of cooperative argumentive dialogue in which the langugae model continuesly prompt the visual-language model

% We proposed a general framework by implementing the Socratic method between a language model and the visual-language model. 

% To mitigate the incomplete and noisy observations returned by the visua 


% The closest work to ours is IPVR~\cite{Chen2023IPVR} despite it superior peroforma it has certain limitations (1). a single-turn visual information query. (2) only focus on knowledge-centric tasks and didn't use diverse visual tools.




==> math_command.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\E}{\mathbb{E}}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

